Tensor-based Collaborative Filtering With Smooth Ratings Scale

Conventional collaborative filtering techniques don't take into consideration the effect of discrepancy in users' rating perception. Some users may rarely give 5 stars to items while others almost always assign 5 stars to the chosen item. Even if they had experience with the same items this systematic discrepancy in their evaluation style will lead to the systematic errors in the ability of recommender system to effectively extract right patterns from data. To mitigate this problem we introduce the ratings' similarity matrix which represents the dependency between different values of ratings on the population level. Hence, if on average the correlations between ratings exist, it is possible to improve the quality of proposed recommendations by off-setting the effect of either shifted down or shifted up users' rates.

==> text/appendicies.tex <==
\section{Appendices}
\label{appendix}


Note that $\widehat{U} \in \mathbb{R}^{M\times r_1}$,
$\widehat{V} \in \mathbb{R}^{N\times r_2}$,
$\widehat{W} \in \mathbb{R}^{K\times r_3}$ 
correspond to the auxiliary latent space. The latent representation of users, items and ratings in the original space is then represented as:

\begin{equation}
\label{eq:orig_latent_1}
%\[
 U = M^{-\frac{1}{2}}\widehat{U}, 
  V = N^{-\frac{1}{2}}\widehat{V},
  W = K^{-\frac{1}{2}}\widehat{W}
%\]
\end{equation}

Columns of the matrices in equation \ref{eq:orig_latent_1} satisfy orthogonality property that is $U^TMU=I_{r_1}, V^TNV=I_{r_2}, W^TKW=I_{r_3} $.


Instead of the 3d case of users-items-rating representation let's consider the 2d case. The standard folding-in technique  for finding a warm-start user representation of his preferences $p^T_0$ is a solution of the following problem:

$$\|p^T_0 - u^T\Sigma V^T\|^2_2 \to min$$

where $u$ is the user latent representation and matrix $V$ is the latent representation of items.

The solution to this minimization problem is

\begin{equation}
\label{eq:u_solution}
u^T = p^T_0 (V^T)^{-1} \Sigma^{-1}
\end{equation}


Obviously, rating prediction is obtained by

\begin{equation}
\label{eq:r_solution}
r^T = u^T \Sigma V^T
\end{equation}

Substituting $V= \widehat{V} = N^\frac{1}{2}V$ to \ref{eq:u_solution} and \ref{eq:r_solution} and using the properties of orthogonality of matrix V, it may be referred that 

\begin{equation}
u^T = p^T_0 ((N^\frac{1}{2}V)^T)^{-1} = p^T_0(N^{-\frac{1}{2}})^TV^{-T}\Sigma^{-1} = p^T_0(N^{-\frac{1}{2}})^TV\Sigma^{-1}
\end{equation}

\begin{equation}
\label{eq:r_pred}
r^T = p^T_0 (N^{-\frac{1}{2}})^TVV^T(N^{\frac{1}{2}})^T
\end{equation}

From \ref{eq:r_pred} it immediately follows that $r = N^{\frac{1}{2}} VV^T N^{-\frac{1}{2}}p_0$. Aggregating the rating prediction of one user for all users we obtain:

\begin{equation}
\label{eq:r_pred_fin}
r = P_0N^{\frac{1}{2}} VV^T N^{-\frac{1}{2}}
\end{equation}

Finally, changing V by W and N by K in \ref{eq:r_pred_fin}  and incorporating it to  \ref{eq:coffee} instead of $WW^T$ (since we are interested in incorporation of similarity just among users leaving $VV^T$ part unchanged) the final formula for prediction is obtained:

\begin{equation}
R_i \approx VV^TP_iK^{\frac{1}{2}}WW^TK^{-\frac{1}{2}}
\end{equation}

==> text/problem.tex <==
\section{Problem Description}
While there are many possible inconsistencies in users' perception this work aims to solve the problem of different perception of the rating scale by users. Consider the following example. For some people giving a 5 star rating to an item is an extraordinary event, they do it rarely and only in exceptional cases. Other users are more generous and most of their ratings are 4 and 5 stars. This leads to a situation where the recommender system treats different ratings as different signals which may be misleading. For example, given two users where the first one rated three last films as 3, 4, 4 and another user rated exactly the same films as 4, 5, 5, we should understand that these are the same sets of preferences. To tackle this problem, this work imposes some notion of similarity. 

